Numerical analysis of parabolic equations with Prandtl--Ishlinskii hysteresis of play type

Rigorous error analysis for numerical approximations of parabolic equations with hysteresis remains limited, even for the widely used Prandtl--Ishlinskii model of play type. In this work, we establish an $O(h+\tau)$ error bound for an implicit Euler $P_1$ finite element discretization. The analysis requires neither higher-order temporal regularity nor additional spatial regularity of the hysteresis variables. For the temporal discretization, we exploit a convex subgradient-flow structure in a weighted Hilbert space and estimates of residual monotone terms to obtain first-order convergence. For the spatial discretization, only the diffusive field is restricted to the finite element space, and a constraint-preserving comparison yields an $O(h)$ semidiscrete estimate. The analysis is developed for play-type Prandtl--Ishlinskii operators formulated directly on a spatial Hilbert space, encompassing the canonical pointwise extension as well as more general spatially structured constraints.

==> Fig/input.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5200.00,3900.00)%
\definecolor{gpBackground}{rgb}{1.000, 1.000, 1.000}%
\put(0,0){\colorbox{gpBackground}{\makebox(5200.00,3900.00)[]{}}}%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,876){\makebox(0,0)[r]{\strut{}-3}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,1325){\makebox(0,0)[r]{\strut{}-2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,1774){\makebox(0,0)[r]{\strut{}-1}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,2223){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,2671){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,3120){\makebox(0,0)[r]{\strut{}2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,3569){\makebox(0,0)[r]{\strut{}3}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(884,541){\makebox(0,0){\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(2912,541){\makebox(0,0){\strut{}0.5}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(4939,541){\makebox(0,0){\strut{}1}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2912,318){\makebox(0,0){\large $t$}}%
      \put(367,2223){\rotatebox{90.00}{\makebox(0,0){\large $u(t)$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,876){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,1325){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,1774){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,2223){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,2671){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,3120){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(764,3569){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(2912,541){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={260.00bp},height={195.00bp}]{input_graphic}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Fig/linear_play.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5200.00,3900.00)%
\definecolor{gpBackground}{rgb}{1.000, 1.000, 1.000}%
\put(0,0){\colorbox{gpBackground}{\makebox(5200.00,3900.00)[]{}}}%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,741){\makebox(0,0)[r]{\strut{}-2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,1482){\makebox(0,0)[r]{\strut{}-1}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2223){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2963){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,3704){\makebox(0,0)[r]{\strut{}2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(884,501){\makebox(0,0){\strut{}-4}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(1898,501){\makebox(0,0){\strut{}-2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(2912,501){\makebox(0,0){\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(3925,501){\makebox(0,0){\strut{}2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(4939,501){\makebox(0,0){\strut{}4}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2912,236){\makebox(0,0){\large $u(t)$}}%
      \put(367,2223){\rotatebox{90.00}{\makebox(0,0){\large $\mathscr{F}_2[u](t)$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,1482){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2223){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2963){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(1898,501){\makebox(0,0){\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(2912,501){\makebox(0,0){\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(3925,501){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={260.00bp},height={195.00bp}]{linear_play_graphic}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Fig/pi_model.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5200.00,3900.00)%
\definecolor{gpBackground}{rgb}{1.000, 1.000, 1.000}%
\put(0,0){\colorbox{gpBackground}{\makebox(5200.00,3900.00)[]{}}}%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,876){\makebox(0,0)[r]{\strut{}-2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,1549){\makebox(0,0)[r]{\strut{}-1}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2223){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2896){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,3569){\makebox(0,0)[r]{\strut{}2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(884,501){\makebox(0,0){\strut{}-4}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(1898,501){\makebox(0,0){\strut{}-2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(2912,501){\makebox(0,0){\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(3925,501){\makebox(0,0){\strut{}2}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(4939,501){\makebox(0,0){\strut{}4}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.00,0.00,0.00}%%
      \put(2912,271){\makebox(0,0){\large $u(t)$}}%
      \put(367,2223){\rotatebox{90.00}{\makebox(0,0){\large $\mathscr{P}[u](t)$}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,876){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,1549){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2223){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,2896){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(740,3569){\makebox(0,0)[r]{\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(1898,501){\makebox(0,0){\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(2912,501){\makebox(0,0){\strut{}}}%
      \colorrgb{0.15,0.15,0.15}%%
      \put(3925,501){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={260.00bp},height={195.00bp}]{pi_model_graphic}}%
    \gplfronttext
  \end{picture}%
\endgroup

